Are Large Language Models Reliable AI Scientists? Assessing Reverse-Engineering of Black-Box Systems

Using AI to create autonomous researchers has the potential to accelerate scientific discovery. A prerequisite for this vision is understanding how well an AI model can identify the underlying structure of a black-box system from its behavior. In this paper, we explore how well a large language model (LLM) learns to identify a black-box function from passively observed versus actively collected data. We investigate the reverse-engineering capabilities of LLMs across three distinct types of black-box systems, each chosen to represent different problem domains where future autonomous AI researchers may have considerable impact: Program, Formal Language, and Math Equation. Through extensive experiments, we show that LLMs fail to extract information from observations, reaching a performance plateau that falls short of the ideal of Bayesian inference. However, we demonstrate that prompting LLMs to not only observe but also intervene -- actively querying the black-box with specific inputs to observe the resulting output -- improves performance by allowing LLMs to test edge cases and refine their beliefs. By providing the intervention data from one LLM to another, we show that this improvement is partly a result of engaging in the process of generating effective interventions, paralleling results in the literature on human learning. Further analysis reveals that engaging in intervention can help LLMs escape from two common failure modes: overcomplication, where the LLM falsely assumes prior knowledge about the black-box, and overlooking, where the LLM fails to incorporate observations. These insights provide practical guidance for helping LLMs more effectively reverse-engineer black-box systems, supporting their use in making new discoveries.

==> figs/ces_overlooking.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{pdf/ces_overlooking.pdf}
       \caption{Overlooking example in math equation black-box}
    \label{fig:ces_overlook}
\end{figure}

==> figs/lang_overcomplication.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{pdf/language_overcomplication.pdf}
    \caption{Overcomplication example in formal language black-box}
    \label{fig:lang_overcomp}
\end{figure}

==> figs/lang_overlooking.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{pdf/language_overlooking.pdf}
    \caption{Overlooking example in formal language black-box}
    \label{fig:lang_overlook}
\end{figure}

==> figs/prog_overcomplication.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{pdf/program_overcomplication.pdf}
    \caption{Overcomplication example in Program black-box}
    \label{fig:prog_overcomp}
\end{figure}

==> figs/two_failures.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=0.8\textwidth]{pdf/two_failures.pdf}
    \caption{Descriptive scores for two different complexity levels. Averaged across three seeds for each of the three black-box types. For math equation, we use descriptive evaluation instead of RMSE only.}
    \label{fig:failures}
\end{figure}




==> sections/research_questions.tex <==
\section{Analysis}
\subsection{Intervention Refines Hypotheses}
\input{figs/intv_effective}

\hc{failure mode should go first?}

Under the O+I setting, the LLM actively tests its own hypotheses during reverse-engineering. As illustrated in Figure \ref{fig:intv_example} (left), in a list-mapping black box instance, GPT-4o designs its next query to evaluate its internal hypothesis by leveraging previously observed valid observations that all input lists return the third integer as the output. This differs from the O-only scenario, where the model can only passively infer patterns from existing data. By actively intervening in the black box, the LLM can iteratively test and refine its hypotheses when failures occur, thereby enhancing the chance to self-verify and reducing the uncertainty of the black box.
In Figure \ref{fig:complexity_gpt4o}, the intervention results for the board game differ from those observed in the other three cases. We hypothesize that for interventions to be effective, the LLM reverse engineering process must obtain additional high-quality information from the interventional data. Specifically, it needs to either (1) test and refine its internal mental model or (2) gather more data to narrow down its uncertainty of the unknown black-box. To accurately reverse engineer the win-loss conditions of a board game, the LLM needs to observe as many end-game cases as possible. However, our deterministic black box uses a greedy strategy for selecting its next actions during O-only sampling. We calculated the average frequency of reaching end-game cases under both O-only and O+I conditions: GPT-4o reaches the end game an average of 10.2  times, compared to only 3.6 times when interventions are involved. This indicates that the failure behavior is mitigated when the LLM reverse engineering process benefits from extra higher-quality data obtained through interventions.

\jy{
\begin{enumerate}
    \item Intv as Obs (more exps; move to analysis?) GPT-4o, 3 seeds
    \item Iterative Hypothesis > Reasoning-only \& hypothesis-only (more exps)
\end{enumerate}
}




\subsection{Two Common Failure Modes: Overcomplication \& Overlooking}
\input{figs/two_failure_modes}
Through extensive experiments across different seeds of the black boxes, we observe that within the same black box type, the effect of the active intervention can vary significantly depending on the complexity of the tasks. In Figure \ref{fig:complexity_gpt4o}, we see that for programs, the intervention yields a 13.9\% improvement on low-complexity instances while only a 1.4\% improvement on high-complexity instances. A similar pattern emerges in formal languages, with a 14.5\% gain on low-complexity instances versus just 0.4\% on high-complexity instances. In contrast, for math equations, the intervention boosts performance by 4.8\% more on high-complexity tasks compared to low-complexity tasks.
Upon delving deeper into black-box complexity, we identify two common failure modes exhibited by GPT4-o in reverse-engineering tasks: (1) overcomplication, where the LLM overinterprets the provided data before formulating a hypothesis about the black box, and (2) overlooking, where the LLM becomes "lazy" in leveraging available information and presents a hypothesis without sufficient reasoning. We categorize these failure behaviors based on whether the LLM effectively utilizes its observations. When GPT-4o fails due to overcomplication, it often performs better on more challenging black box instances, likely because those black boxes demand more in-depth reasoning. However, when GPT-4o overlooks information, it tends to form a more accurate internal mental model for low-complexity black boxes, where failing to use all available data does not significantly impair performance.

==> tables/task_complexity.tex <==
\newcommand{\numplain}[2][2.8em]{\makebox[#1][r]{#2}}        
\newcommand{\numdelta}[3][2.8em]{\makebox[#1][r]{#2}$_{\color{red}{#3}}$} 

\begin{table*}[ht]
\centering
\setlength{\tabcolsep}{6pt}  
\renewcommand{\arraystretch}{1.15} 
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccc}
\toprule
           & easy & easy\_medium & medium & medium\_hard & hard & Avg \\ \midrule

\rowcolor{gray!20}\multicolumn{7}{l}{\textbf{Programs}}\\
Observation  & \(42.2\) & \(55.6\) & \(29.7\) & \(20.8\) & \(81.9\) & \(46.0\) \\
Intervention & \numdelta{\(54.9\)}{+12.7} & \numdelta{\(59.6\)}{+4.0} & 
       \numdelta{\(31.4\)}{+1.7} & \numdelta{\(21.6\)}{+0.8} & 
       \numdelta{\(81.3\)}{-0.6} & \numdelta{\(49.8\)}{+3.8} \\ \addlinespace[2pt]

\rowcolor{gray!20}\multicolumn{7}{l}{\textbf{Formal Languages}}\\
Observation & \(36.2\) & -- & \(16.7\) & -- & \(21.3\) & \(24.7\) \\
intv & \numdelta{\(48.3\)}{+12.1} & -- & 
       \numdelta{\(24.7\)}{+8.0} & -- & 
       \numdelta{\(29.8\)}{+8.5} & \numdelta{\(34.3\)}{+9.6} \\ \addlinespace[2pt]

\rowcolor{gray!20}\multicolumn{7}{l}{\textbf{Math Equations}}\\
Observation & \(33.7\) & \(33.2\) & \(29.8\) & \(32.5\) & \(25.7\) & \(31.0\) \\
Intervention & \numdelta{\(42.0\)}{+8.3} & \numdelta{\(35.2\)}{+2.0} & 
       \numdelta{\(36.5\)}{+6.7} & \numdelta{\(40.3\)}{+7.8} & 
       \numdelta{\(35.1\)}{+9.4} & \numdelta{\(37.8\)}{+6.8} \\ 
\bottomrule
\end{tabular*}
\end{table*}




